IRS: An Incentive-compatible Reward Scheme for Algorand

Founded in 2017, Algorand is one of the world's first carbon-negative, public blockchains inspired by proof of stake. Algorand uses a Byzantine agreement protocol to add new blocks to the blockchain. The protocol can tolerate malicious users as long as a supermajority of the stake is controlled by non-malicious users. The protocol achieves about 100x more throughput compared to Bitcoin and can be easily scaled to millions of nodes. Despite its impressive features, Algorand lacks a reward-distribution scheme that can effectively incentivize nodes to participate in the protocol. In this work, we study the incentive issue in Algorand through the lens of game theory. We model the Algorand protocol as a Bayesian game and propose a novel reward scheme to address the incentive issue in Algorand. We derive necessary conditions to ensure that participation in the protocol is a Bayesian Nash equilibrium under our proposed reward scheme even in the presence of a malicious adversary. We also present quantitative analysis of our proposed reward scheme by applying it to two real-world deployment scenarios. We estimate the costs of running an Algorand node and simulate the protocol to measure the overheads in terms of computation, storage, and networking.

==> Sections/6-referral.tex <==
\section{Expected Rewards under \name}
\label{sec:referral}

In \refsec{sec:analysis}, we showed that cooperating is a BNE strategy for non-Byzantine agents under the \name reward scheme.
In this section, we study expected rewards gained by Byzantine and non-Byzantine nodes.
If there is no adversary (i.e., $p_b = 0$), then in equilibrium, all agents receive the same expected rewards under \name according to \reflemm{lemm:expected-utility} and \refthm{thm:BNEByzantine}.
However, in the presence of an adversary, \name could fail to provide proportional rewards.
This is mainly because \name relies on selected agents to refer cooperation of other agents.
Non-Byzantine agents refer both Byzantine and non-Byzantine agents.
Byzantine agents, however, do not refer non-Byzantine agents.
If we assume that Byzantine agents do refer other Byzantine agents, then the adversary has the opportunity to receive a higher expected reward per Byzantine agent than non-Byzantine agents%
\footnote{This could be achieved when, for example, the adversary code fully mimics the protocol except referring the cooperation  of the other agents.}.
This could pose a risk to Algorand as the expected proportion of assets controlled by the adversary could increase under \name.

\subsection{Referral Mechanism}
To prevent corrupted nodes to receive higher expected rewards than non-corrupted nodes, we propose a referral reward mechanism.
Under this mechanism, selected committee members receive extra rewards for every agent that they refer in their vote.
More specifically, for every agent that is referred in a committee member's vote, the committee member receives a referral reward of $ R^r(k) / \vert \hat{N}_i \vert $, where $R^r(k)$ is a fixed referral reward at step $k$.
The addition of referral rewards poses a dilemma for the adversary.
If a Byzantine agent propagates messages to its non-Byzantine peers, it gains expected baseline rewards but enables non-Byzantine agents to claim referral rewards.
Similarly, if a Byzantine committee member refers its non-Byzantine neighbors, it gains referral rewards, but that allows non-Byzantine agents to gain baseline rewards.
In the remainder of this section, we consider four cases for the adversary code: (I) does not propagate messages to non-Byzantine peers but refers all neighbors, (II) does not propagate messages to non-Byzantine peers and only refers Byzantine neighbors, (III) propagates messages to all peers but only refers Byzantine neighbors, and (IV) propagates messages to all peers and refers all neighbors.

The total reward of agent $i$ given action profile $a$ and type vector $\theta$ with referral rewards can be formulated as:
\[
R_i(a, \theta) = \sum_{k = 1}^{K(a, \theta)} R_i^b(a, \theta, k) + R_i^c(a, \theta, k) + R_i^r(a, \theta, k).
\]
Here, $R_i^c(a, \theta, k) = R^c(k) \times \II(\theta_{i,k} \le p_c)$ for all four cases.
% $R_i^b(a, \theta, k)$ is defined for each case as follows.
% \[
% \scriptstyle
% R_i^b(a, \theta, k) =
% \begin{cases}
% (R^{b}(k) / n_{rs}) \sum_{j \in N_i} \II(\theta_{j,k} \le p_c, a_j \in \{C, M\}) & \text{for (I)/(IV) if } \theta_{i,0} = 0, \\
% (R^{b}(k) / n_{rs}) \sum_{j \in N_i} \II(\theta_{j,k} \le p_c, a_j = C) &\text{for (II)/(III) if } \theta_{i,0} = 0,\\
% (R^{b}(k) / n_{rs}) \sum_{j \in N_i} \II(\theta_{j,k} \le p_c, a_j \in \{C, M\}) & \text{for (III)/(IV) if } \theta_{i,0} = 1,\\
% (R^{b}(k) / n_{rs}) \sum_{j \in N_i} \II(\theta_{j,k} \le p_c, a_j = M)& \text{for (I)/(II) if } \theta_{i,0} = 1.\\
% \end{cases}
% \]
For cases (I) and (IV), Byzantine committee members refer all their neighbors.
Therefore, if $\theta_{i,0} = 0$, then agent $i$ receives baseline rewards for being referred by any cooperating or misbehaving peer that is selected as a committee member.
For cases (II) and (III), Byzantine committee members only refer their Byzantine neighbors.
This means that if $\theta_{i,0} = 0$, then agent $i$ receives baseline rewards only for being referred by cooperating committee members among its peers.
For cases (III) and (IV), Byzantine agents propagate messages to all their peers.
Therefore, if $\theta_{i,0} = 1$, agent $i$ receives baseline rewards for being referred by any cooperating or misbehaving peer that is selected as a committee member. 
Finally, for cases (I) and (II), Byzantine agents do not propagate messages to their non-Byzantine peers.
For these two cases, if $\theta_{i,0} = 1$, agent $i$ receives baseline rewards for being referred by misbehaving committee members among its neighbors.

Similarly,
% $R_i^r(a, \theta, k)$ is defined as follows.
% \[
% \scriptstyle
% R_i^r(a, \theta, k) =
% \begin{cases}
% (R^{r}(k) / \vert \hat{N}_i \vert) \sum_{j \in \hat{N}_i} \II(\theta_{i,k} \le p_c, a_j = C) &\text{for (I)/(II) if } \theta_{i,0} = 0, \\
% (R^{r}(k) / \vert \hat{N}_i \vert) \sum_{j \in \hat{N}_i} \II(\theta_{i,k} \le p_c, a_j \in \{C, M\}) &\text{for (III)/(IV) if } \theta_{i,0} = 0, \\
% (R^{r}(k) / \vert \hat{N}_i \vert) \sum_{j \in \hat{N}_i} \II(\theta_{i,k} \le p_c) &\text{for (I)/(IV) if } \theta_{i,0} = 1, \\
% (R^{r}(k) / \vert \hat{N}_i \vert) \sum_{j \in \hat{N}_i} \II(\theta_{i,k} \le p_c, \theta_{j,0} = 1) &\text{for (II)/(III) if } \theta_{i,0} = 1.
% \end{cases}
% \]
for cases (I) and (II), Byzantine agents only propagate messages to their Byzantine neighbors.
Therefore, if $\theta_{i,0} = 0$, then committee member $i$ can only claim referral rewards for cooperating peers.
For cases (III) and (IV), Byzantine agents propagate messages to all their neighbors.
This means that if $\theta_{i,0} = 0$, then committee member $i$ receives referral rewards for referring any cooperating or misbehaving peer.
For cases (I) and (IV), Byzantine agents refer all their neighbors.
Therefore, if $\theta_{i,0} = 1$, committee member  $i$ receives referral rewards for all its neighbors.
Finally, for cases (II) and (III), Byzantine agents only refer their Byzantine neighbors.
For these two cases, if $\theta_{i,0} = 1$, committee member $i$ only claims referral rewards for its Byzantine neighbors.

We next formulate conditional expectation of rewards.
\begin{lemma}
\label{lemm:expected-rewards}
Consider any agent $i$.
Suppose that the strategy profile of all agents except agent $i$ is $s_{-i}^*$ where for each agent $j \in N \setminus i$, if $\theta_{j,0} = 0$, then $s_j^*(C \given \theta_j) = 1$, and $s_j^*(M \given \theta_j) = 1$ otherwise.
Suppose further that agent $i$ adopts strategy $s_i$ which plays $M$ if $\theta_{i,0} = 1$ and plays $C$ with probability $s_c$ and $D$ with probability $1 - s_c$ if $\theta_{i,0} = 0$.
Let $a^*(\theta)$ be an action profile where $a^*_i$ is $C$ if $\theta_{i,0} = 0$ and $M$ otherwise.
Define $K(\theta) = K(a^*(\theta), \theta)$.
Under \name with referral rewards, the conditional expectation of agent $i$'s reward given $\theta_{i,0} = 0$ is:
\[
\EX_{a,\theta}[R_i(a, \theta) \given \theta_{i,0} = 0] = s_c \; \sum_{\ell=1}^{\kmax} \EP(K(\theta) = \ell) \sum_{k=1}^{\ell} \bar{R}(k),
\]
where $\bar{R}(k)$ is defined as:
\[
\scriptstyle
\bar{R}(k) = 
\begin{cases}
R^b(k) \; p_c + R^c(k) \; p_c + R^r(k) \; p_c \; (1 - p_b) &\text{for (I)},\\
R^b(k) \; p_c \; (1 - p_b) + R^c(k) \; p_c + R^r(k) \; p_c \; (1 - p_b) &\text{for (II)},\\
R^b(k) \; p_c \; (1 - p_b) + R^c(k) \; p_c + R^r(k) \; p_c &\text{for (III)},\\
R^b(k) \; p_c + R^c(k) \; p_c + R^r(k) \; p_c &\text{for (IV)}.
\end{cases}
\]
Similarly, the conditional expectation of agent $i$'s reward given $\theta_{i,0} = 1$ is:
\[
\EX_{a,\theta}[R_i(a, \theta) \given \theta_{i,0} = 1] = \sum_{\ell=1}^{\kmax} \EP(K(\theta) = \ell) \sum_{k=1}^{\ell} \bar{R}_b(k),
\]
where $\bar{R}_b(k)$ is defined as:
\[
\bar{R}_b(k) = 
\begin{cases}
R^b(k) \; p_c \; p_b + R^c(k) \; p_c + R^r(k) \; p_c &\text{for (I)},\\
R^b(k) \; p_c \; p_b + R^c(k) \; p_c + R^r(k) \; p_c \; p_b &\text{for (II)},\\
R^b(k) \; p_c + R^c(k) \; p_c + R^r(k) \; p_c \; p_b &\text{for (III)},\\
R^b(k) \; p_c + R^c(k) \; p_c + R^r(k) \; p_c &\text{for (IV)}.
\end{cases}
\]
\end{lemma}

The proof is deferred to the appendix (see \refapp{app:referral-proofs}).
Given the expected rewards, we formulate the expected utility of each agent in the following lemma.

\begin{lemma}
\label{lemm:expected-utilities-with-referral}
Consider any agent $i$.
Suppose that the strategy profile of all agents except agent $i$ is $s_{-i}^*$ where for each agent $j \in N \setminus i$, if $\theta_{j,0} = 0$, then $s_j^*(C \given \theta_j) = 1$, and $s_j^*(M \given \theta_j) = 1$ otherwise.
Suppose further that agent $i$ adopts strategy $s_i$ which plays $M$ if $\theta_{i,0} = 1$ and plays $C$ with probability $s_c$ and $D$ with probability $1 - s_c$ if $\theta_{i,0} = 0$.
Let $a^*(\theta)$ be an action profile where $a^*_i$ is $C$ if $\theta_{i,0} = 0$ and $M$ otherwise.
Define $K(\theta) = K(a^*(\theta), \theta)$.
Under \name with referral rewards, the expected utility of agent $i$ is:
\begin{align*}
& \EU_i((s_i, s^*_{-i})) \\
= & s_c \; (1 - p_b) \; \sum_{\ell=1}^{\kmax} \EP(K(\theta) = \ell) \sum_{k=1}^{\ell} \bar{R}(k) - \bar{C}^b(k) - C^c(k) \; p_c,
\end{align*}
where $\bar{R}(k)$ is defined similar to \reflemm{lemm:expected-rewards}.
\end{lemma}

\begin{proof}
Using the same techniques in the proof of \reflemm{lemm:expected-utility}, we can write:
\begin{align*}
\label{equ:utility-rewrite}
\EU_i&((s_i, s^*_{-i})) = \EX_{\theta}\left[\sum_{k=1}^{K(\theta)} u_{i}(a^*(\theta), \theta, k) \given[\Big] \theta_{i,0} = 0\right] \\
= &\sum_{\ell=1}^{\kmax} \sum_{k=1}^{\ell} \EP(K(\theta) = \ell) \\
& \; \EX_{\theta}\left[R_i(a^*(\theta), \theta, k) - C_i(a^*(\theta), \theta, k) \given \theta_{i,0} = 0, K(\theta) = \ell\right].
\end{align*}
Substituting conditional expectation of rewards from \reflemm{lemm:expected-rewards} and conditional expectation of costs from \refequ{equ:expected-costs} completes the proof.
\end{proof}

Given the two lemmas, we next prove that cooperation is a BNE strategy for non-Byzantine agents under \name with referral rewards under certain conditions.
\begin{theorem}
\label{thm:BNEByzantine-cases}
Let $s^*$ be a strategy profile where for each agent $i$, if $\theta_{i,0} = 0$, then $s_i^*(C \given \theta_i) = 1$, and otherwise, $s_i^*(M \given \theta_i) = 1$.
Given $p_c$, $p_b$, $\bar{C}^b(k)$, and $C^c(k)$ for  $k = 1, \dots, \kmax$, $s^*$ is a BNE under \name with referral rewards if for $k = 1, \dots, \kmax$:
\[
R^b(k) \; (1 - p_b) + R^c(k) + R^r(k) \; (1 - p_b) \ge \bar{C}^b(k) / p_c + C^c(k)
% ,  ~~ \forall k = 1, \dots, \kmax
.
\]
\end{theorem}

\begin{proof}
For $\bar{R}(k)$ defined in \reflemm{lemm:expected-rewards}, it is easy to show that for all four cases and for $k = 1, \dots, \kmax$:
\[
\bar{R}(k) \ge R^b(k) \; p_c \; (1 - p_b) + R^c(k) \; p_c + R^r(k) \; p_c \; (1 - p_b)
% ,  ~~ \forall k = 1, \dots, \kmax
.
\]
Therefore, the condition of the theorem implies:
\[
\bar{R}(k) - \bar{C}^b(k) + C^c(k) \; p_c \ge 0.
\]
Consequently, $\EU_i((s_i, s^*_{-i}))$ is maximized when $s_c = 1$.
In this case, we have $s = s^*$ which means $s^*$ is a BNE.
\end{proof}

Finally, we show that Byzantine agents cannot gain more expected rewards under \name with referral rewards than non-Byzantine agents for all four cases when certain conditions on referral and baseline rewards are met.
\begin{theorem}
\label{thm:antitrust}
Let $s^*$ be a strategy profile where for each agent $i$, if $\theta_{i,0} = 0$, then $s_i^*(C \given \theta_i) = 1$, and otherwise, $s_i^*(M \given \theta_i) = 1$.
Under \name, with the referral reward mechanism, the expected reward of each Byzantine agent for strategy profile $s^*$ is less than or equal to that of non-Byzantine agents if for $k = 1, \dots, \kmax$:
\[
R^b(k) \; (1-p_b) \ge R^r(k) \; p_b \text{ and } R^r(k) \; (1-p_b) \ge R^b(k) \; p_b
% , ~~ \forall k = 1, \dots, \kmax
.
\]
\end{theorem}

\begin{proof}
Given \reflemm{lemm:expected-rewards}, to ensure that the expected reward of any Byzantine agent is less than or equal to that of non-Byzantine agents (i.e. $\EX_{a,\theta}[R_i(a, \theta) \given \theta_{i,0} = 0] \ge \EX_{a,\theta}[R_i(a, \theta) \given \theta_{i,0} = 1]$), all the following four inequalities must hold for $k = 1, \dots, \kmax$.
\begin{itemize}
 \item $R^b(k) + R^r(k) \; (1 - p_b) \ge R^b(k) \; p_b + R^r(k)$,
 \item $R^b(k) \; (1 - p_b) + R^r(k) \; (1 - p_b) \ge R^b(k) \; p_b + R^r(k) \; p_b$,
 \item $R^b(k) \; (1 - p_b) + R^r(k) \ge R^b(k) + R^r(k) \; p_b$, and
 \item $R^b(k) + R^r(k) \ge R^b(k) + R^r(k)$.
\end{itemize}
The first inequality (corresponding to case (I)) can be simplified as $R^b(k) (1-p_b) \ge R^r(k) p_b$.
The second inequality (corresponding to case (II)) always holds since $0 \le p_b < 1/3$.
The third inequality (corresponding to case (III)) can be written as $R^r(k) (1-p_b) \ge R^b(k) p_b$.
Finally, the fourth inequality (corresponding to case (IV)) always holds.
\end{proof}


==> rebuttal_WG.tex <==
[long intro]
We agree. We will revise the intro.

[1/2 vs 1/3]
Our paper assumes for analysis of rewards that the environment is synchronous. However, Algorand itself does not require strong synchrony and can only tolerate < 1/3 Byzantine nodes. We adopt the same resilience threshold for consistency with the Algorand protocol because we borrow Theorem 1 from [15] (Algorand paper) in the proof of Proposition 5.

[K_max]
To produce a block, the Algorand protocol runs at most for K_max steps. However, a block could be generated much earlier. Appendix D summarizes each step of the Algorand protocol. Once the protocol terminates, a block is generated (the second if statement in Alg. 1). If consensus is not reached by K_max steps, a recovery mechanism is put in motion (e.g., to resolve a fork). This is outside the scope of our analysis due to our synchrony assumption.

[Byzantine agents not including non-Byzantine agents in votes]
This assumption is made to calculate a lower bound on the expected utility of non-Byzantine agents. In other words, if the condition of Theorem 7 is met, then non-Byzantine agents are incentivized to participate even if Byzantine agents do not include the identity of non-Byzantine agents. If Byzantine agents include the identity of non-Byzantine agents, the expected utility of non-Byzantine agents can only increase, and this does not break our incentives analysis. We will clarify this in the text.

We agree with Reviewer 1 that if Byzantine agents do not include identities of non-Byzantine agents, then on average they report 2/3 less identities. However, when agents do not participate as committee members very often, short-term measurements (e.g., a single vote) do not yield observations that could be reliably used to identify Byzantine agents.

[Dependence of strategies on types]
The type vector has multiple elements. The first element of the type vector identifies whether an agent is compromised by the adversary. The remaining elements identify whether an agent is selected as a committee member at different steps. By definition, non-Byzantine agents are not compromised by the adversary. For the equilibrium analysis, we show that cooperation of non-Byzantine agents does not depend on the other elements of their type vector.

[Intuition for BNE condition]
The expected rewards should outweigh the expected costs. The condition in Theorem 7 is mainly derived from the expected utility calculated in Lemma 6. Agents receive R_b if their neighbors are selected as a committee member (w.p. p_c) and are not corrupted (w.p. 1-p_b). Further, agents receive R_c if they are selected as a committee member (w.p. p_c). Agents pay a baseline cost under all circumstances and pay a committee cost only when they are selected as a committee. Concrete values for reward parameters are discussed in Sec. 7.1. We will add further explanation to the text.

[Overhead of including identities in votes]
In Section 7.2 we discuss the expected storage overhead (~8KB). This means that each committee member will have to include on average an additional 8KB of data in each vote.

[Rewards: 20 vs several thousand Algos]
First, we note that most blocks are generated within the first 5 steps. This means that for most blocks, no reward is given for steps 6 to K_max. Second, for the reward calculation in Sec. 7.2, we assume that each agent has a single sub-node. This is a worst-case analysis because unlike expected rewards, expected costs do not necessarily increase linearly as a function of sub-nodes. As mentioned in Sec. 7.2, in the real-world deployment of Algorand, each agent has on average 40 million sub-nodes. To use IRS in practice, one might modify the parameters of the analysis to only consider agents with a certain minimum number of sub-nodes (e.g., 1 million sub-nodes). In such settings, incurred costs per sub-node will dramatically decrease, and as a result, the necessary rewards will be close to the current rewards. Finally, in real-world settings, some agents are altruistic (i.e., they participate in the protocol regardless of the rewards). Inclusion of such agents in the analysis would lead to lower rewards. Extending IRS to include altruistic agents would be an interesting future work, both theoretically and in practice.

[Incentives in Ethereum’s Hybrid Casper Protocol]
We will add this paper to the related work.

[Centralized vs distributed reward scheme]
Designing a decentralized reward scheme is an interesting future work. What makes designing such schemes challenging is the presence of the adversary. A decentralized reward distribution scheme should be resilient to scenarios where Byzantine agents are selected to distribute the reward.

[Effect on carbon-negativity]
In terms of computation, as discussed in Sec. 7.2, IRS adds 17% overhead. This overhead can be reduced by limiting the frequency of network reconstruction. Regarding networking and storage, ISR has limited carbon footprint because networking and storage are energy disproportional (i.e., the energy consumption does not proportionally change as a function of network/storage utilization). We will add more details with regard to this point to the text.

[Justification for assumptions]
In earlier sections of this rebuttal, we have provided some intuition for some our assumptions. We would be happy to add/provide more details for any specific assumption that the reviewers point out.

